Detection of adrenal anomalous findings in spinal CT images using multi model graph aggregation

Low back pain is the symptom that is the second most frequently reported to primary care physicians, effecting 50 to 80 percent of the population in a lifetime, resulting in multiple referrals of patients suffering from back problems, to CT and MRI scans, which are then examined by radiologists. The radiologists examining these spinal scans naturally focus on spinal pathologies and might miss other types of abnormalities, and in particular, abdominal ones, such as malignancies. Nevertheless, the patients whose spine was scanned might as well have malignant and other abdominal pathologies. Thus, clinicians have suggested the need for computerized assistance and decision support in screening spinal scans for additional abnormalities. In the current study, We have addressed the important case of detecting suspicious lesions in the adrenal glands as an example for the overall methodology we have developed. A patient CT scan is integrated from multiple slices with an axial orientation. Our method determines whether a patient has an abnormal adrenal gland, and localises the abnormality if it exists. Our method is composed of three deep learning models; each model has a different task for achieving the final goal. We call our compound method the Multi Model Graph Aggregation MMGA method. The novelty in this study is twofold. First, the use, for an important screening task, of CT scans that are originally focused and tuned for imaging the spine, which were acquired from patients with potential spinal disorders, for detection of a totally different set of abnormalities such as abdominal Adrenal glands pathologies. Second, we have built a complex pipeline architecture composed from three deep learning models that can be utilized for other organs (such as the pancreas or the kidney), or for similar applications, but using other types of imaging, such as MRI.

==> Future.tex <==
In the following section we provide few directions for potential future work that can leverage our MMGA method.

\subsection{Integrate Reject Option - SelectiveNet}
The main idea is enabling the model to reject prediction on the hard cases that their confidence level is lower than others, this method is called by the author Yonatan Geifman "SelectiveNet"~\cite{geifman2019selectivenet}. This can give a big benefit to the system, by allowing the model to say "I don't know" for a predefined percentage of samples, by that the the accuracy improves and the tough cases will be directed to Radiologists attention to give more careful prediction, which the system can collect them for future learning on the hard cases.

The SelectiveNet is trained to optimize both classification (or regression) and rejection simultaneously (the rejection trained together with the entire network). A selective model is basically a pair $(f,g)$ where $f$ is a prediction function and $g:\chi \rightarrow \{0,1\}$ is a selection function, which serves as a binary qualifier for $f$ as follows:

\begin{equation}
(f,g)(x) =
\begin{cases}
f(x) & \text{if } g(x)=1 \\
\text{don't know} & \text{if } g(x)=0 \\
\end{cases}
\end{equation}


\subsection{Multi-modal learning - Combining CT and MRI scans}

A good direction is to examine how to combine different data types such as CT and MRI scans into a single model in a way that will harness the connections between CT and MRI so that eventually improve accuracy against a single scan type model. Existing studies in the field of automatically detecting pathologies from scans are based on a \textit{single} input type of images, such as CT scans, and do not consider other types of inputs such as MRI, due to the limited availability of paired MR-CT data. Thus, a good objective is to examine whether a system that can harness information from  paired CT-MR scans and perform a classification of a possible anomaly in the abdominal areas, might be better than a system using only one type of imaging.

% Another important aspect that medicine and patients can benefit from, is the comprehension of the differences between CT to MRI cans with respect to the resolution of the information captured in the image. As known CT scan is much cheaper and more available to the public than MRI, and MRI is considered the imaging method of choice in assessing the extent of bone and soft-tissue tumors~\cite{aisen1986mri}. Thus harnessing the gap between CT and MRI scans will enable us to use this knowledge when there is no MRI available or has very long waiting line. Eventually this knowledge should increase the accuracy of CT scan only diagnosis,
% or in other words learning the connections between CT and MRI scans and using them in order to obtain a better CT scan only based model. The motivation behind this idea is to take advantage of the MRI scans which are better for some cases, more scarce and harder to get. Using a model where there are only CT scans available which is relevant to majority of the patients can increase the accuracy. One direction method is to take late fusion alike model, detach the MRI CNN related and retrain the CT scan Network latter layers for classification and localization tasks. By doing so the early layers are fixed that where achieved during training together with MRI scans possibly reflect the correlation between CT and MRI scans that can help the CT scan only model to use this correlation for achieving better results. 



% Multi-modal learning is typically performed with network architectures containing modality-specific layers and shared layers, utilizing co-registered images of different modalities~\cite{dou2020unpaired} such as MRI and CT. A common practice is to develop a quantitative assessment for similar analysis via segmentation method, e.g., a convolutional neural network (CNN), separately for CT and MRI data. Such separate training leaves potentially valuable cross-modality information unused. Qi Dou et al.,~\cite{dou2020unpaired} propose a novel learning scheme for unpaired cross-modality image segmentation using CT and MRI scans, with a highly compact architecture achieving superior segmentation accuracy. In his method, they heavily reuse network parameters, by sharing all convolutional kernels across CT and MRI, and only employ modality-specific internal normalization layers which compute respective statistics.
% \plan{Show picture of scheme}

% Another work in the field of Multi-Modal learning but as apposed to previous one it uses same image types as co-registered images, they are pairs of MRI scans. As images are easy to access in medical images and they usually contain complementary information. So well utilizing multi-modal images in tumor detection is always an important and valuable research topic~\cite{pan2021liver}. 

% Modern object detection frameworks are mainly based on
% Convolution Neural Network (CNN) .Most of them only
% take single-modal images, making them not able to utilize the
% complementary information of different modalities. Early fusion and late fusion are two simple solutions to achieve multi-modal object detection. For early fusion, in Fig. \ref{fig:intermediate}(a), the original images are integrated directly as the input of the network. Nevertheless, it does not consider the correlation between different modal features. In contrast, the late fusion, in Fig. \ref{fig:intermediate}(b), extracts features of each modality through two independent networks and then combines the high-level feature maps.

% \begin{figure}[!h]
%     \centering
%     \includegraphics[scale=0.75]{Pictures/IntermediateFusion.png}
%     \caption{Early/Late and novel intermediate fusion schemes}
%     \label{fig:intermediate}
% \end{figure}
% Chao Pan et al.,~\cite{pan2021liver} developed a novel multi-scale intermediate multi-modal fusion detection framework to achieve multi-modal liver tumor detection.
% Unlike early or late fusion, it maintains two branches of different modal information and introduces cross-modal feature interaction progressively, thus better leveraging the complementary information contained in multi-modalities. Fig. \ref{fig:intermediate} visualizes the differences between classical late/early fusion to the intermediate fusion.


==> Plan.tex <==
\textbf{\textit{Plan}}

\noindent The following are the main milestones in the research: 
\begin{enumerate}
\item Medical data acquiring 
\item Labeling the data by Experts
\item Pre-process CT and MRI scans
\item Developing the CT scans model
\item Developing the MRI scans model
\item Developing the Combined CT and MRI model
\item Developing the Detached model for CT scans
\item Draft the results and discussion chapters
\item Writing an article

\end{enumerate}
\textbf{\textit{Time line}}

\noindent A Gantt timeline chart was designed to establish rough timeline of all activities for next year. This is to ensure all activities are completed within the agreed time frame. Please refer to the following Gantt Chart and Schedule:
\begin{figure}[!h]
\centering
\includegraphics[scale=0.612]{Pictures/Schedule.png}
\caption{Proposed Research Schedule}
\label{fig:PRS}
\end{figure}


==> ResearchGoal.tex <==
\subsection{Overall Research Aim}
This research examine different Deep Learning methods of supervised learning with emphasis on a Medical CT Scans as an input data. The aim of these methods is to detect and classify abdominal cancerous pathologies.

% \subsection{Research Questions}
% The following research questions will be applied to this area of study:
% \begin{enumerate}
% \item Can we use CT scans that are directed and tuned for the spine which were taken from patients with back issues, and use them for diagnosing different illnesses such as abdominal pathologies.
% \item Is it possible to detect and classify abdominal pathologies from CT and MRI spinal scans, using CNN networks and deep learning methods?
% % \item Can we achieve most or all of the accuracy of an MRI scan model, when interpreted by a human, using a CT scan  model augmented by Deep Learning?
% \item What is the contribution of using both CT and MRI, compared to using each of them alone? 
% \item What is the contribution of adding patient data to each of the following three options - CT, MRI, CT \& MRI?
% \end{enumerate}

\subsection{Implication Of The Research}
\begin{enumerate}
    \item  
    Building a system that gets as input CT scans that are directed and tuned for the spine and which were taken from patients with back issues, and using it for automatically detecting different illnesses such as Adrenal pathologies, can significantly assist radiologists in interpreting spinal scans,  reduce False Negative diagnostic results, and enhance the safety of patients.
    % \item Building a system that can harness information from multiple types of imaging scans, in particular, CT and MRI, might enhance the accuracy of detecting anomalies in the abdominal areas, compared to the use of only one imaging mode.
    \item 
    Is it possible to detect and classify Adrenal pathologies from CT spinal scans, using CNN networks and deep learning methods?
    \item 
    Creating a generic recipe for building unique 3 fold pipeline can benefit to whole other organs anomaly detection not restricted to abdominal area and CT scans.
    \item 
    Creating a method supporting simultaneously multiple organs detection .i.e a single model detecting both left and right anomalous adrenals.
    \item 
    Can final aggregation step in pipeline which predicts whether patient's entire scan has abnormal Adrenal can be simplified form Graph learning complex method to a simple rule based method achieving same or better performance.
    
\end{enumerate}



==> cover_heb.tex <==

\begin{titlepage}
    \begin{center}
        \vspace*{1cm}
        
        \includegraphics[width=0.1\textwidth]{Pictures/BGU_lable.png}\\
        \selectlanguage{hebrew}אוניברסיטת בן-גוריון בנגב\\הפקולטה למדעי הטבע\\המחלקה למדעי המחשב\selectlanguage{english}

        \vspace{2cm}
        
        \selectlanguage{hebrew}
        {\Large \thesistitlehe}
        \selectlanguage{english}
        
        \vspace{1.5cm}

        \selectlanguage{hebrew}
        חיבור זה מהווה חלק מהדרישות לקבלת התואר מוסמך למדעי הטבע\selectlanguage{english}(M.Sc)
        \vspace{1cm}
        
        \selectlanguage{hebrew}
        \thesisauthornamehe
        \selectlanguage{english}
        \vspace{1cm}

        \selectlanguage{hebrew}
        בהנחיית \thesissupervisernamehe 
        \selectlanguage{english}
        
        \vfill
        \selectlanguage{hebrew}
        \thesismonthhe \quad
        \selectlanguage{english}
        \thesisyear
     \end{center}
\end{titlepage}

==> cover_page.tex <==
\begin{titlepage}
    \begin{center}
        \vspace*{1cm}
        
        \includegraphics[width=0.1\textwidth]{Pictures/BGU_lable.png}\\
        Ben-Gurion University of the Negev\\
        The Faculty of Engineering Sciences\\
        Department of Software and Information Systems Engineering
        
        \vspace{2cm}
        
        {\Large \thesistitle}
        
        \vspace{1cm}
        
        Thesis submitted in partial fulfillment of the requirements\\for the Master of Sciences degree
        
        \vspace{1cm}
        
        By: \thesisauthorname
        
        \vspace{1cm}
        
        Under the supervision of \thesissupervisername
        
        \vfill
        
        \thesismonth \quad \thesisyear

    \end{center}
\end{titlepage}

==> title_page.tex <==
\begin{titlepage}
    \begin{center}
        \vspace*{1cm}
        
        \includegraphics[width=0.1\textwidth]{Pictures/BGU_lable.png}\\
        Ben-Gurion University of the Negev\\
        The Faculty of Engineering Sciences\\
        Department of Software and Information Systems Engineering
        
        \vspace{1cm}
        
        {\Large \thesistitle}
        
        \vspace{0.5cm}
        
        Thesis submitted in partial fulfillment of the requirements\\for the Master of Sciences degree
        
        \vspace{0.5cm}
        
        \thesisauthorname
        
        \vspace{0.5cm}
        
        Under the supervision of \thesissupervisername
        
        \vspace{0.5cm}
        
        \begin{flushleft}
        Signature of student: \( \rule{3cm}{0.15mm} \) \hfill Date: \( \rule{3cm}{0.15mm} \)\\
        Signature of supervisor: \( \rule{3cm}{0.15mm} \) \hfill Date: \( \rule{3cm}{0.15mm} \)\\
        Signature of chairperson of the\\committee for graduate studies: \( \rule{3cm}{0.15mm} \) \hfill Date: \( \rule{3cm}{0.15mm} \)
        \end{flushleft}
        
        \vfill
        
        \thesismonth \quad \thesisyear
    \end{center}
\end{titlepage}
